Computing in the fractal cloud: modular generic solvers for SAT and Q-SAT variants

Abstract geometrical computation can solve hard combinatorial problems efficiently: we showed previously how Q-SAT can be solved in bounded space and time using instance-specific signal machines and fractal parallelization. In this article, we propose an approach for constructing a particular generic machine for the same task. This machine deploies the Map/Reduce paradigm over a fractal structure. Moreover our approach is modular: the machine is constructed by combining modules. In this manner, we can easily create generic machines for solving satifiability variants, such as SAT, #SAT, MAX-SAT.

==> Fig_New/fig___2011_ICALP_corridors.tex <==
\def\Zone(#1)(#2)(#3)(#4){\draw[fill,fill=purple,thick,fill opacity=0.5,draw=green!50!black](#1)--(#2)--(#3)--(#4);}%
\Zone(8.75,9.12)(8.75,12.12)(9.375,12.745)(9.375,9.745)%
\Zone(8.75,9.12)(8.75,12.12)(8.125,12.745)(8.125,9.745)%
\Zone(6.25,9.12)(6.25,12.12)(6.875,12.745)(6.875,9.745)%
\Zone(6.25,9.12)(6.25,12.12)(5.625,12.745)(5.625,9.745)%
\Zone(7.5,7.87)(7.5,10.870000000000001)(8.75,12.120000000000001)(8.75,9.120000000000001)%
\Zone(7.5,7.87)(7.5,10.870000000000001)(6.25,12.120000000000001)(6.25,9.120000000000001)%
\Zone(3.75,9.12)(3.75,12.12)(4.375,12.745)(4.375,9.745)%
\Zone(3.75,9.12)(3.75,12.12)(3.125,12.745)(3.125,9.745)%
\Zone(1.25,9.12)(1.25,12.12)(1.875,12.745)(1.875,9.745)%
\Zone(1.25,9.12)(1.25,12.12)(0.625,12.745)(0.625,9.745)%
\Zone(2.5,7.87)(2.5,10.870000000000001)(3.75,12.120000000000001)(3.75,9.120000000000001)%
\Zone(2.5,7.87)(2.5,10.870000000000001)(1.25,12.120000000000001)(1.25,9.120000000000001)%
\Zone(5.0,5.37)(5.0,8.370000000000001)(7.5,10.870000000000001)(7.5,7.87)%
\Zone(5.0,5.37)(5.0,8.370000000000001)(2.5,10.870000000000001)(2.5,7.87)%
\Zone(0.0,0.37)(0.0,3.37)(5.0,8.370000000000001)(5.0,5.37)%


==> Fig_New/fig___2011_ICALP_corridors_lenses.tex <==
\def\Zone(#1)(#2)(#3)(#4)(#5){\draw[fill,fill=purple,thick,fill opacity=0.5,draw=green!50!black](#1)--(#2)--(#3)--(#4) -- (#5);}%
\Zone(8.75,9.12)(8.75,9.495)(9.09375,9.83875)(9.375,9.9325)(9.375,9.745)%
\Zone(8.75,9.12)(8.75,9.495)(8.40625,9.83875)(8.125,9.9325)(8.125,9.745)%
\Zone(6.25,9.12)(6.25,9.495)(6.59375,9.83875)(6.875,9.9325)(6.875,9.745)%
\Zone(6.25,9.12)(6.25,9.495)(5.90625,9.83875)(5.625,9.9325)(5.625,9.745)%
\Zone(7.5,7.87)(7.5,8.620000000000001)(8.1875,9.307500000000001)(8.75,9.495000000000001)(8.75,9.120000000000001)%
\Zone(7.5,7.87)(7.5,8.620000000000001)(6.8125,9.307500000000001)(6.25,9.495000000000001)(6.25,9.120000000000001)%
\Zone(3.75,9.12)(3.75,9.495)(4.09375,9.83875)(4.375,9.9325)(4.375,9.745)%
\Zone(3.75,9.12)(3.75,9.495)(3.40625,9.83875)(3.125,9.9325)(3.125,9.745)%
\Zone(1.25,9.12)(1.25,9.495)(1.59375,9.83875)(1.875,9.9325)(1.875,9.745)%
\Zone(1.25,9.12)(1.25,9.495)(0.90625,9.83875)(0.625,9.9325)(0.625,9.745)%
\Zone(2.5,7.87)(2.5,8.620000000000001)(3.1875,9.307500000000001)(3.75,9.495000000000001)(3.75,9.120000000000001)%
\Zone(2.5,7.87)(2.5,8.620000000000001)(1.8125,9.307500000000001)(1.25,9.495000000000001)(1.25,9.120000000000001)%
\Zone(5.0,5.37)(5.0,6.87)(6.375,8.245000000000001)(7.5,8.620000000000001)(7.5,7.87)%
\Zone(5.0,5.37)(5.0,6.87)(3.625,8.245000000000001)(2.5,8.620000000000001)(2.5,7.87)%
\Zone(0.0,0.37)(0.0,3.37)(2.75,6.12)(5.0,6.87)(5.0,5.37)%


==> Fig_New/fig___2011_ICALP_sig_def.tex <==
%\usepackage{denys}

%% key   label   color
\newColorRGB{KOLORAllL}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{AllL}{$\ST\sigforallL$}{KOLORAllL}
\newColorRGB{KOLORAllR}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{AllR}{$\ST\sigforallR$}{KOLORAllR}
\newColorRGB{KOLORConjL}{0.60784316}{0.078431375}{0.6156863}
\tikzAGCmakeSignal{ConjL}{$\LLO\sigand$}{KOLORConjL}
\newColorRGB{KOLORConjLL}{0.60784316}{0.078431375}{0.6156863}
\tikzAGCmakeSignal{ConjLL}{$\LHI\sigand$}{KOLORConjLL}
\newColorRGB{KOLORConjR}{0.60784316}{0.078431375}{0.6156863}
\tikzAGCmakeSignal{ConjR}{$\RLO\sigand$}{KOLORConjR}
\newColorRGB{KOLORConjRR}{0.60784316}{0.078431375}{0.6156863}
\tikzAGCmakeSignal{ConjRR}{$\RHI\sigand$}{KOLORConjRR}
\newColorRGB{KOLORDisjL}{0.9647059}{0.54509807}{0.003921569}
\tikzAGCmakeSignal{DisjL}{$\LLO\sigor$}{KOLORDisjL}
\newColorRGB{KOLORDisjLL}{0.9647059}{0.54509807}{0.003921569}
\tikzAGCmakeSignal{DisjLL}{$\LHI\sigor$}{KOLORDisjLL}
\newColorRGB{KOLORDisjR}{0.9647059}{0.54509807}{0.003921569}
\tikzAGCmakeSignal{DisjR}{$\RLO\sigor$}{KOLORDisjR}
\newColorRGB{KOLORDisjRR}{0.9647059}{0.54509807}{0.003921569}
\tikzAGCmakeSignal{DisjRR}{$\RHI\sigor$}{KOLORDisjRR}
\newColorRGB{KOLORFalse}{0.95686275}{0.03137255}{0.03137255}
\tikzAGCmakeSignal{False}{$\ST\sigF$}{KOLORFalse}
\newColorRGB{KOLORFalseL}{0.95686275}{0.03137255}{0.03137255}
\tikzAGCmakeSignal{FalseL}{$\LLO\sigF$}{KOLORFalseL}
\newColorRGB{KOLORFalseLL}{0.95686275}{0.03137255}{0.03137255}
\tikzAGCmakeSignal{FalseLL}{$\LHI\sigF$}{KOLORFalseLL}
\newColorRGB{KOLORFalseR}{0.95686275}{0.03137255}{0.03137255}
\tikzAGCmakeSignal{FalseR}{$\RLO\sigF$}{KOLORFalseR}
\newColorRGB{KOLORFalseRR}{0.95686275}{0.03137255}{0.03137255}
\tikzAGCmakeSignal{FalseRR}{$\RHI\sigF$}{KOLORFalseRR}
\newColorRGB{KOLORNegL}{0.5568628}{0.34901962}{0.08235294}
\tikzAGCmakeSignal{NegL}{$\LLO\signot$}{KOLORNegL}
\newColorRGB{KOLORNegLL}{0.5568628}{0.34901962}{0.08235294}
\tikzAGCmakeSignal{NegLL}{$\LHI\signot$}{KOLORNegLL}
\newColorRGB{KOLORNegR}{0.5568628}{0.34901962}{0.08235294}
\tikzAGCmakeSignal{NegR}{$\RLO\signot$}{KOLORNegR}
\newColorRGB{KOLORNegRR}{0.5568628}{0.34901962}{0.08235294}
\tikzAGCmakeSignal{NegRR}{$\RHI\signot$}{KOLORNegRR}
\newColorRGB{KOLOROneL}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{OneL}{$\ST\sigexistsL$}{KOLOROneL}
\newColorRGB{KOLOROneR}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{OneR}{$\ST\sigexistsR$}{KOLOROneR}
\newColorRGB{KOLORTrue}{0.0}{1.0}{0.0}
\tikzAGCmakeSignal{True}{$\ST\sigT$}{KOLORTrue}
\newColorRGB{KOLORTrueL}{0.0}{1.0}{0.0}
\tikzAGCmakeSignal{TrueL}{$\LLO\sigT$}{KOLORTrueL}
\newColorRGB{KOLORTrueLL}{0.0}{1.0}{0.0}
\tikzAGCmakeSignal{TrueLL}{$\LHI\sigT$}{KOLORTrueLL}
\newColorRGB{KOLORTrueR}{0.0}{1.0}{0.0}
\tikzAGCmakeSignal{TrueR}{$\RLO\sigT$}{KOLORTrueR}
\newColorRGB{KOLORTrueRR}{0.0}{1.0}{0.0}
\tikzAGCmakeSignal{TrueRR}{$\RHI\sigT$}{KOLORTrueRR}
\newColorRGB{KOLORa}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{a}{$\ST\sigstart$}{KOLORa}
\newColorRGB{KOLORaL}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{aL}{$\LLO\sigstart$}{KOLORaL}
\newColorRGB{KOLORaLL}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{aLL}{$\LHI\sigstart$}{KOLORaLL}
\newColorRGB{KOLORaR}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{aR}{$\RLO\sigstart$}{KOLORaR}
\newColorRGB{KOLORaRR}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{aRR}{$\RHI\sigstart$}{KOLORaRR}
\newColorRGB{KOLORallL}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{allL}{$\LLO\sigforall$}{KOLORallL}
\newColorRGB{KOLORallLL}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{allLL}{$\LHI\sigforall$}{KOLORallLL}
\newColorRGB{KOLORallR}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{allR}{$\RLO\sigforall$}{KOLORallR}
\newColorRGB{KOLORallRR}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{allRR}{$\RHI\sigforall$}{KOLORallRR}
\newColorRGB{KOLORalphaL}{0.9882353}{1.0}{0.15294118}
\tikzAGCmakeSignal{alphaL}{$\LLO\sigstartaux$}{KOLORalphaL}
\newColorRGB{KOLORalphaLL}{0.9882353}{1.0}{0.15294118}
\tikzAGCmakeSignal{alphaLL}{$\LHI\sigstartaux$}{KOLORalphaLL}
\newColorRGB{KOLORalphaR}{0.9882353}{1.0}{0.15294118}
\tikzAGCmakeSignal{alphaR}{$\RLO\sigstartaux$}{KOLORalphaR}
\newColorRGB{KOLORalphaRR}{0.9882353}{1.0}{0.15294118}
\tikzAGCmakeSignal{alphaRR}{$\RHI\sigstartaux$}{KOLORalphaRR}
\newColorRGB{KOLORaoff}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{aoff}{$\ST\sigstartoff$}{KOLORaoff}
\newColorRGB{KOLORaoffL}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{aoffL}{$\LLO\sigstartoff$}{KOLORaoffL}
\newColorRGB{KOLORaoffLL}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{aoffLL}{$\LHI\sigstartoff$}{KOLORaoffLL}
\newColorRGB{KOLORaoffR}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{aoffR}{$\RLO\sigstartoff$}{KOLORaoffR}
\newColorRGB{KOLORaoffRR}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{aoffRR}{$\RHI\sigstartoff$}{KOLORaoffRR}
\newColorRGB{KOLORbetaL}{0.4392157}{0.9098039}{0.7607843}
\tikzAGCmakeSignal{betaL}{$\LLO\sigxdelay$}{KOLORbetaL}
\newColorRGB{KOLORbetaLL}{0.4392157}{0.9098039}{0.7607843}
\tikzAGCmakeSignal{betaLL}{$\LHI\sigxdelay$}{KOLORbetaLL}
\newColorRGB{KOLORbetaR}{0.4392157}{0.9098039}{0.7607843}
\tikzAGCmakeSignal{betaR}{$\RLO\sigxdelay$}{KOLORbetaR}
\newColorRGB{KOLORbetaRR}{0.4392157}{0.9098039}{0.7607843}
\tikzAGCmakeSignal{betaRR}{$\RHI\sigxdelay$}{KOLORbetaRR}
\newColorRGB{KOLORcollectL}{0.039215688}{0.3254902}{0.019607844}
\tikzAGCmakeSignal{collectL}{$\LLO\sigcollect$}{KOLORcollectL}
\newColorRGB{KOLORcollectLL}{0.039215688}{0.3254902}{0.019607844}
\tikzAGCmakeSignal{collectLL}{$\LHI\sigcollect$}{KOLORcollectLL}
\newColorRGB{KOLORcollectR}{0.039215688}{0.3254902}{0.019607844}
\tikzAGCmakeSignal{collectR}{$\RLO\sigcollect$}{KOLORcollectR}
\newColorRGB{KOLORcollectRR}{0.039215688}{0.3254902}{0.019607844}
\tikzAGCmakeSignal{collectRR}{$\RHI\sigcollect$}{KOLORcollectRR}
\newColorRGB{KOLORconjL}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{conjL}{$\LLO\sigandZ$}{KOLORconjL}
\newColorRGB{KOLORconjLL}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{conjLL}{$\LHI\sigandZ$}{KOLORconjLL}
\newColorRGB{KOLORconjR}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{conjR}{$\RLO\sigandZ$}{KOLORconjR}
\newColorRGB{KOLORconjRR}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{conjRR}{$\RHI\sigandZ$}{KOLORconjRR}
\newColorRGB{KOLORdisjL}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{disjL}{$\LLO\sigorZ$}{KOLORdisjL}
\newColorRGB{KOLORdisjLL}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{disjLL}{$\LHI\sigorZ$}{KOLORdisjLL}
\newColorRGB{KOLORdisjR}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{disjR}{$\RLO\sigorZ$}{KOLORdisjR}
\newColorRGB{KOLORdisjRR}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{disjRR}{$\RHI\sigorZ$}{KOLORdisjRR}
\newColorRGB{KOLORfL}{0.60784316}{0.078431375}{0.6156863}
\tikzAGCmakeSignal{fL}{$\LLO\sigfP$}{KOLORfL}
\newColorRGB{KOLORfLL}{0.60784316}{0.078431375}{0.6156863}
\tikzAGCmakeSignal{fLL}{$\LHI\sigfP$}{KOLORfLL}
\newColorRGB{KOLORfR}{0.60784316}{0.078431375}{0.6156863}
\tikzAGCmakeSignal{fR}{$\RLO\sigfP$}{KOLORfR}
\newColorRGB{KOLORfRR}{0.60784316}{0.078431375}{0.6156863}
\tikzAGCmakeSignal{fRR}{$\RHI\sigfP$}{KOLORfRR}
\newColorRGB{KOLORfalse}{0.95686275}{0.03137255}{0.03137255}
\tikzAGCmakeSignal{false}{$\ST\sigf$}{KOLORfalse}
\newColorRGB{KOLORfalseL}{0.95686275}{0.03137255}{0.03137255}
\tikzAGCmakeSignal{falseL}{$\LLO\sigf$}{KOLORfalseL}
\newColorRGB{KOLORfalseLL}{0.95686275}{0.03137255}{0.03137255}
\tikzAGCmakeSignal{falseLL}{$\LHI\sigf$}{KOLORfalseLL}
\newColorRGB{KOLORfalseR}{0.95686275}{0.03137255}{0.03137255}
\tikzAGCmakeSignal{falseR}{$\RLO\sigf$}{KOLORfalseR}
\newColorRGB{KOLORfalseRR}{0.95686275}{0.03137255}{0.03137255}
\tikzAGCmakeSignal{falseRR}{$\RHI\sigf$}{KOLORfalseRR}
\newColorRGB{KOLORgammaL}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{gammaL}{$\LLO\siggammaP$}{KOLORgammaL}
\newColorRGB{KOLORgammaLL}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{gammaLL}{$\LHI\siggammaP$}{KOLORgammaLL}
\newColorRGB{KOLORgammaR}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{gammaR}{$\RLO\siggammaP$}{KOLORgammaR}
\newColorRGB{KOLORgammaRR}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{gammaRR}{$\RHI\siggammaP$}{KOLORgammaRR}
\newColorRGB{KOLORgammaoffL}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{gammaoffL}{$\LLO\siggamma$}{KOLORgammaoffL}
\newColorRGB{KOLORgammaoffLL}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{gammaoffLL}{$\LLHI\siggamma$}{KOLORgammaoffLL}
\newColorRGB{KOLORgammaoffR}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{gammaoffR}{$\RLO\siggamma$}{KOLORgammaoffR}
\newColorRGB{KOLORgammaoffRR}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{gammaoffRR}{$\RHI\siggamma$}{KOLORgammaoffRR}
\newColorRGB{KOLORidcL}{0.60784316}{0.078431375}{0.6156863}
\tikzAGCmakeSignal{idcL}{$\LLO\sigandP$}{KOLORidcL}
\newColorRGB{KOLORidcLL}{0.60784316}{0.078431375}{0.6156863}
\tikzAGCmakeSignal{idcLL}{$\LHI\sigandP$}{KOLORidcLL}
\newColorRGB{KOLORidcR}{0.60784316}{0.078431375}{0.6156863}
\tikzAGCmakeSignal{idcR}{$\RLO\sigandP$}{KOLORidcR}
\newColorRGB{KOLORidcRR}{0.60784316}{0.078431375}{0.6156863}
\tikzAGCmakeSignal{idcRR}{$\RHI\sigandP$}{KOLORidcRR}
\newColorRGB{KOLORiddL}{0.9647059}{0.54509807}{0.003921569}
\tikzAGCmakeSignal{iddL}{$\LLO\sigorP$}{KOLORiddL}
\newColorRGB{KOLORiddLL}{0.9647059}{0.54509807}{0.003921569}
\tikzAGCmakeSignal{iddLL}{$\LHI\sigorP$}{KOLORiddLL}
\newColorRGB{KOLORiddR}{0.9647059}{0.54509807}{0.003921569}
\tikzAGCmakeSignal{iddR}{$\RLO\sigorP$}{KOLORiddR}
\newColorRGB{KOLORiddRR}{0.9647059}{0.54509807}{0.003921569}
\tikzAGCmakeSignal{iddRR}{$\RHI\sigorP$}{KOLORiddRR}
\newColorRGB{KOLORnegL}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{negL}{$\LLO\signotZ$}{KOLORnegL}
\newColorRGB{KOLORnegLL}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{negLL}{$\LHI\signotZ$}{KOLORnegLL}
\newColorRGB{KOLORnegR}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{negR}{$\RLO\signotZ$}{KOLORnegR}
\newColorRGB{KOLORnegRR}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{negRR}{$\RHI\signotZ$}{KOLORnegRR}
\newColorRGB{KOLORoneL}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{oneL}{$\LLO\sigexists$}{KOLORoneL}
\newColorRGB{KOLORoneLL}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{oneLL}{$\LHI\sigexists$}{KOLORoneLL}
\newColorRGB{KOLORoneR}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{oneR}{$\RLO\sigexists$}{KOLORoneR}
\newColorRGB{KOLORoneRR}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{oneRR}{$\RHI\sigexists$}{KOLORoneRR}
\newColorRGB{KOLORstoreL}{0.4392157}{0.9098039}{0.7607843}
\tikzAGCmakeSignal{storeL}{$\LLO\sigs$}{KOLORstoreL}
\newColorRGB{KOLORstoreLL}{0.4392157}{0.9098039}{0.7607843}
\tikzAGCmakeSignal{storeLL}{$\LHI\sigs$}{KOLORstoreLL}
\newColorRGB{KOLORstoreR}{0.4392157}{0.9098039}{0.7607843}
\tikzAGCmakeSignal{storeR}{$\RLO\sigs$}{KOLORstoreR}
\newColorRGB{KOLORstoreRR}{0.4392157}{0.9098039}{0.7607843}
\tikzAGCmakeSignal{storeRR}{$\RHI\sigs$}{KOLORstoreRR}
\newColorRGB{KOLORtL}{0.9647059}{0.54509807}{0.003921569}
\tikzAGCmakeSignal{tL}{$\LLO\sigtP$}{KOLORtL}
\newColorRGB{KOLORtLL}{0.9647059}{0.54509807}{0.003921569}
\tikzAGCmakeSignal{tLL}{$\LHI\sigtP$}{KOLORtLL}
\newColorRGB{KOLORtR}{0.9647059}{0.54509807}{0.003921569}
\tikzAGCmakeSignal{tR}{$\RLO\sigtP$}{KOLORtR}
\newColorRGB{KOLORtRR}{0.9647059}{0.54509807}{0.003921569}
\tikzAGCmakeSignal{tRR}{$\RHI\sigtP$}{KOLORtRR}
\newColorRGB{KOLORtrue}{0.0}{1.0}{0.0}
\tikzAGCmakeSignal{true}{$\ST\sigt$}{KOLORtrue}
\newColorRGB{KOLORtrueL}{0.0}{1.0}{0.0}
\tikzAGCmakeSignal{trueL}{$\LLO\sigt$}{KOLORtrueL}
\newColorRGB{KOLORtrueLL}{0.0}{1.0}{0.0}
\tikzAGCmakeSignal{trueLL}{$\LHI\sigt$}{KOLORtrueLL}
\newColorRGB{KOLORtrueR}{0.0}{1.0}{0.0}
\tikzAGCmakeSignal{trueR}{$\RLO\sigt$}{KOLORtrueR}
\newColorRGB{KOLORtrueRR}{0.0}{1.0}{0.0}
\tikzAGCmakeSignal{trueRR}{$\RHI\sigt$}{KOLORtrueRR}
\newColorRGB{KOLORw}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{w}{$\ST\sigwall$}{KOLORw}
\newColorRGB{KOLORx}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{x}{$\ST\sigx$}{KOLORx}
\newColorRGB{KOLORxL}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{xL}{$\LLO\sigx$}{KOLORxL}
\newColorRGB{KOLORxLL}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{xLL}{$\LHI\sigx$}{KOLORxLL}
\newColorRGB{KOLORxR}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{xR}{$\RLO\sigx$}{KOLORxR}
\newColorRGB{KOLORxRR}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{xRR}{$\RHI\sigx$}{KOLORxRR}
\newColorRGB{KOLORxoff}{0.4392157}{0.9098039}{0.7607843}
\tikzAGCmakeSignal{xoff}{$\ST\sigxoff$}{KOLORxoff}
\newColorRGB{KOLORzL}{0.95686275}{0.03137255}{0.03137255}
\tikzAGCmakeSignal{zL}{$\LLO\sigstop$}{KOLORzL}
\newColorRGB{KOLORzLL}{0.95686275}{0.03137255}{0.03137255}
\tikzAGCmakeSignal{zLL}{$\LHI\sigstop$}{KOLORzLL}
\newColorRGB{KOLORzR}{0.95686275}{0.03137255}{0.03137255}
\tikzAGCmakeSignal{zR}{$\RLO\sigstop$}{KOLORzR}
\newColorRGB{KOLORzRR}{0.95686275}{0.03137255}{0.03137255}
\tikzAGCmakeSignal{zRR}{$\RHI\sigstop$}{KOLORzRR}
\newColorRGB{KOLORzetaL}{0.99215686}{0.16470589}{0.7490196}
\tikzAGCmakeSignal{zetaL}{$\LLO\sigstopaux$}{KOLORzetaL}
\newColorRGB{KOLORzetaLL}{0.99215686}{0.16470589}{0.7490196}
\tikzAGCmakeSignal{zetaLL}{$\LHI\sigstopaux$}{KOLORzetaLL}
\newColorRGB{KOLORzetaR}{0.99215686}{0.16470589}{0.7490196}
\tikzAGCmakeSignal{zetaR}{$\RLO\sigstopaux$}{KOLORzetaR}
\newColorRGB{KOLORzetaRR}{0.99215686}{0.16470589}{0.7490196}
\tikzAGCmakeSignal{zetaRR}{$\RHI\sigstopaux$}{KOLORzetaRR}

==> Fig_New/fig___2011_ICALP_sig_defOK.tex <==
%\usepackage{denys}

%% key   label   color
\newColorRGB{KOLORAllL}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{AllL}{$\ST\sigforallL$}{KOLORAllL}
\newColorRGB{KOLORAllR}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{AllR}{$\ST\sigforallR$}{KOLORAllR}
\newColorRGB{KOLORConjL}{0.60784316}{0.078431375}{0.6156863}
\tikzAGCmakeSignal{ConjL}{$\LLO\sigand$}{KOLORConjL}
\newColorRGB{KOLORConjLL}{0.60784316}{0.078431375}{0.6156863}
\tikzAGCmakeSignal{ConjLL}{$\LHI\sigand$}{KOLORConjLL}
\newColorRGB{KOLORConjR}{0.60784316}{0.078431375}{0.6156863}
\tikzAGCmakeSignal{ConjR}{$\RLO\sigand$}{KOLORConjR}
\newColorRGB{KOLORConjRR}{0.60784316}{0.078431375}{0.6156863}
\tikzAGCmakeSignal{ConjRR}{$\RHI\sigand$}{KOLORConjRR}
\newColorRGB{KOLORDisjL}{0.9647059}{0.54509807}{0.003921569}
\tikzAGCmakeSignal{DisjL}{$\LLO\sigor$}{KOLORDisjL}
\newColorRGB{KOLORDisjLL}{0.9647059}{0.54509807}{0.003921569}
\tikzAGCmakeSignal{DisjLL}{$\LHI\sigor$}{KOLORDisjLL}
\newColorRGB{KOLORDisjR}{0.9647059}{0.54509807}{0.003921569}
\tikzAGCmakeSignal{DisjR}{$\RLO\sigor$}{KOLORDisjR}
\newColorRGB{KOLORDisjRR}{0.9647059}{0.54509807}{0.003921569}
\tikzAGCmakeSignal{DisjRR}{$\RHI\sigor$}{KOLORDisjRR}
\newColorRGB{KOLORFalse}{0.95686275}{0.03137255}{0.03137255}
\tikzAGCmakeSignal{False}{$\ST\sigF$}{KOLORFalse}
\newColorRGB{KOLORFalseL}{0.95686275}{0.03137255}{0.03137255}
\tikzAGCmakeSignal{FalseL}{$\LLO\sigF$}{KOLORFalseL}
\newColorRGB{KOLORFalseLL}{0.95686275}{0.03137255}{0.03137255}
\tikzAGCmakeSignal{FalseLL}{$\LHI\sigF$}{KOLORFalseLL}
\newColorRGB{KOLORFalseR}{0.95686275}{0.03137255}{0.03137255}
\tikzAGCmakeSignal{FalseR}{$\RLO\sigF$}{KOLORFalseR}
\newColorRGB{KOLORFalseRR}{0.95686275}{0.03137255}{0.03137255}
\tikzAGCmakeSignal{FalseRR}{$\RHI\sigF$}{KOLORFalseRR}
\newColorRGB{KOLORNegL}{0.5568628}{0.34901962}{0.08235294}
\tikzAGCmakeSignal{NegL}{$\LLO\signot$}{KOLORNegL}
\newColorRGB{KOLORNegLL}{0.5568628}{0.34901962}{0.08235294}
\tikzAGCmakeSignal{NegLL}{$\LHI\signot$}{KOLORNegLL}
\newColorRGB{KOLORNegR}{0.5568628}{0.34901962}{0.08235294}
\tikzAGCmakeSignal{NegR}{$\RLO\signot$}{KOLORNegR}
\newColorRGB{KOLORNegRR}{0.5568628}{0.34901962}{0.08235294}
\tikzAGCmakeSignal{NegRR}{$\RHI\signot$}{KOLORNegRR}
\newColorRGB{KOLOROneL}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{OneL}{$\ST\sigexistsL$}{KOLOROneL}
\newColorRGB{KOLOROneR}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{OneR}{$\ST\sigexistsR$}{KOLOROneR}
\newColorRGB{KOLORTrue}{0.0}{1.0}{0.0}
\tikzAGCmakeSignal{True}{$\ST\sigT$}{KOLORTrue}
\newColorRGB{KOLORTrueL}{0.0}{1.0}{0.0}
\tikzAGCmakeSignal{TrueL}{$\LLO\sigT$}{KOLORTrueL}
\newColorRGB{KOLORTrueLL}{0.0}{1.0}{0.0}
\tikzAGCmakeSignal{TrueLL}{$\LHI\sigT$}{KOLORTrueLL}
\newColorRGB{KOLORTrueR}{0.0}{1.0}{0.0}
\tikzAGCmakeSignal{TrueR}{$\RLO\sigT$}{KOLORTrueR}
\newColorRGB{KOLORTrueRR}{0.0}{1.0}{0.0}
\tikzAGCmakeSignal{TrueRR}{$\RHI\sigT$}{KOLORTrueRR}
\newColorRGB{KOLORa}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{a}{$\ST\sigstart$}{KOLORa}
\newColorRGB{KOLORaL}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{aL}{$\LLO\sigforall$}{KOLORaL}
\newColorRGB{KOLORaLL}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{aLL}{$\LHI\sigforall$}{KOLORaLL}
\newColorRGB{KOLORaR}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{aR}{$\RLO\sigforall$}{KOLORaR}
\newColorRGB{KOLORaRR}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{aRR}{$\RHI\sigforall$}{KOLORaRR}
\newColorRGB{KOLORallL}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{allL}{$\LLO\sigforall$}{KOLORallL}
\newColorRGB{KOLORallLL}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{allLL}{$\LHI\sigforall$}{KOLORallLL}
\newColorRGB{KOLORallR}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{allR}{$\RLO\sigforall$}{KOLORallR}
\newColorRGB{KOLORallRR}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{allRR}{$\RHI\sigforall$}{KOLORallRR}
\newColorRGB{KOLORalphaL}{0.9882353}{1.0}{0.15294118}
\tikzAGCmakeSignal{alphaL}{$\LLO\sigstartaux$}{KOLORalphaL}
\newColorRGB{KOLORalphaLL}{0.9882353}{1.0}{0.15294118}
\tikzAGCmakeSignal{alphaLL}{$\LHI\sigstartaux$}{KOLORalphaLL}
\newColorRGB{KOLORalphaR}{0.9882353}{1.0}{0.15294118}
\tikzAGCmakeSignal{alphaR}{$\RLO\sigstartaux$}{KOLORalphaR}
\newColorRGB{KOLORalphaRR}{0.9882353}{1.0}{0.15294118}
\tikzAGCmakeSignal{alphaRR}{$\RHI\sigstartaux$}{KOLORalphaRR}
\newColorRGB{KOLORaoff}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{aoff}{$\ST\sigstartoff$}{KOLORaoff}
\newColorRGB{KOLORaoffL}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{aoffL}{$\LLO\sigstartoff$}{KOLORaoffL}
\newColorRGB{KOLORaoffLL}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{aoffLL}{$\LHI\sigstartoff$}{KOLORaoffLL}
\newColorRGB{KOLORaoffR}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{aoffR}{$\RLO\sigstartoff$}{KOLORaoffR}
\newColorRGB{KOLORaoffRR}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{aoffRR}{$\RHI\sigstartoff$}{KOLORaoffRR}
\newColorRGB{KOLORbetaL}{0.4392157}{0.9098039}{0.7607843}
\tikzAGCmakeSignal{betaL}{$\LLO\sigxdelay$}{KOLORbetaL}
\newColorRGB{KOLORbetaLL}{0.4392157}{0.9098039}{0.7607843}
\tikzAGCmakeSignal{betaLL}{$\LHI\sigxdelay$}{KOLORbetaLL}
\newColorRGB{KOLORbetaR}{0.4392157}{0.9098039}{0.7607843}
\tikzAGCmakeSignal{betaR}{$\RLO\sigxdelay$}{KOLORbetaR}
\newColorRGB{KOLORbetaRR}{0.4392157}{0.9098039}{0.7607843}
\tikzAGCmakeSignal{betaRR}{$\RHI\sigxdelay$}{KOLORbetaRR}
\newColorRGB{KOLORcollectL}{0.039215688}{0.3254902}{0.019607844}
\tikzAGCmakeSignal{collectL}{$\LLO\sigcollect$}{KOLORcollectL}
\newColorRGB{KOLORcollectLL}{0.039215688}{0.3254902}{0.019607844}
\tikzAGCmakeSignal{collectLL}{$\LHI\sigcollect$}{KOLORcollectLL}
\newColorRGB{KOLORcollectR}{0.039215688}{0.3254902}{0.019607844}
\tikzAGCmakeSignal{collectR}{$\RLO\sigcollect$}{KOLORcollectR}
\newColorRGB{KOLORcollectRR}{0.039215688}{0.3254902}{0.019607844}
\tikzAGCmakeSignal{collectRR}{$\RHI\sigcollect$}{KOLORcollectRR}
\newColorRGB{KOLORconjL}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{conjL}{$\LLO\sigandZ$}{KOLORconjL}
\newColorRGB{KOLORconjLL}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{conjLL}{$\LHI\sigandZ$}{KOLORconjLL}
\newColorRGB{KOLORconjR}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{conjR}{$\RLO\sigandZ$}{KOLORconjR}
\newColorRGB{KOLORconjRR}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{conjRR}{$\RHI\sigandZ$}{KOLORconjRR}
\newColorRGB{KOLORdisjL}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{disjL}{$\LLO\sigorZ$}{KOLORdisjL}
\newColorRGB{KOLORdisjLL}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{disjLL}{$\LHI\sigorZ$}{KOLORdisjLL}
\newColorRGB{KOLORdisjR}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{disjR}{$\RLO\sigorZ$}{KOLORdisjR}
\newColorRGB{KOLORdisjRR}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{disjRR}{$\RHI\sigorZ$}{KOLORdisjRR}
\newColorRGB{KOLORfL}{0.60784316}{0.078431375}{0.6156863}
\tikzAGCmakeSignal{fL}{$\LLO\sigfP$}{KOLORfL}
\newColorRGB{KOLORfLL}{0.60784316}{0.078431375}{0.6156863}
\tikzAGCmakeSignal{fLL}{$\LHI\sigfP$}{KOLORfLL}
\newColorRGB{KOLORfR}{0.60784316}{0.078431375}{0.6156863}
\tikzAGCmakeSignal{fR}{$\RLO\sigfP$}{KOLORfR}
\newColorRGB{KOLORfRR}{0.60784316}{0.078431375}{0.6156863}
\tikzAGCmakeSignal{fRR}{$\RHI\sigfP$}{KOLORfRR}
\newColorRGB{KOLORfalse}{0.95686275}{0.03137255}{0.03137255}
\tikzAGCmakeSignal{false}{$\ST\sigf$}{KOLORfalse}
\newColorRGB{KOLORfalseL}{0.95686275}{0.03137255}{0.03137255}
\tikzAGCmakeSignal{falseL}{$\LLO\sigf$}{KOLORfalseL}
\newColorRGB{KOLORfalseLL}{0.95686275}{0.03137255}{0.03137255}
\tikzAGCmakeSignal{falseLL}{$\LHI\sigf$}{KOLORfalseLL}
\newColorRGB{KOLORfalseR}{0.95686275}{0.03137255}{0.03137255}
\tikzAGCmakeSignal{falseR}{$\RLO\sigf$}{KOLORfalseR}
\newColorRGB{KOLORfalseRR}{0.95686275}{0.03137255}{0.03137255}
\tikzAGCmakeSignal{falseRR}{$\RHI\sigf$}{KOLORfalseRR}
\newColorRGB{KOLORgammaL}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{gammaL}{$\LLO\siggammaP$}{KOLORgammaL}
\newColorRGB{KOLORgammaLL}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{gammaLL}{$\LHI\siggammaP$}{KOLORgammaLL}
\newColorRGB{KOLORgammaR}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{gammaR}{$\RLO\siggammaP$}{KOLORgammaR}
\newColorRGB{KOLORgammaRR}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{gammaRR}{$\RHI\siggammaP$}{KOLORgammaRR}
\newColorRGB{KOLORgammaoffL}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{gammaoffL}{$\LLO\siggamma$}{KOLORgammaoffL}
\newColorRGB{KOLORgammaoffLL}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{gammaoffLL}{$\LLHI\siggamma$}{KOLORgammaoffLL}
\newColorRGB{KOLORgammaoffR}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{gammaoffR}{$\RLO\siggamma$}{KOLORgammaoffR}
\newColorRGB{KOLORgammaoffRR}{0.68235296}{0.65882355}{0.65882355}
\tikzAGCmakeSignal{gammaoffRR}{$\RHI\siggamma$}{KOLORgammaoffRR}
\newColorRGB{KOLORidcL}{0.60784316}{0.078431375}{0.6156863}
\tikzAGCmakeSignal{idcL}{$\LLO\sigandP$}{KOLORidcL}
\newColorRGB{KOLORidcLL}{0.60784316}{0.078431375}{0.6156863}
\tikzAGCmakeSignal{idcLL}{$\LHI\sigandP$}{KOLORidcLL}
\newColorRGB{KOLORidcR}{0.60784316}{0.078431375}{0.6156863}
\tikzAGCmakeSignal{idcR}{$\RLO\sigandP$}{KOLORidcR}
\newColorRGB{KOLORidcRR}{0.60784316}{0.078431375}{0.6156863}
\tikzAGCmakeSignal{idcRR}{$\RHI\sigandP$}{KOLORidcRR}
\newColorRGB{KOLORiddL}{0.9647059}{0.54509807}{0.003921569}
\tikzAGCmakeSignal{iddL}{$\LLO\sigorP$}{KOLORiddL}
\newColorRGB{KOLORiddLL}{0.9647059}{0.54509807}{0.003921569}
\tikzAGCmakeSignal{iddLL}{$\LHI\sigorP$}{KOLORiddLL}
\newColorRGB{KOLORiddR}{0.9647059}{0.54509807}{0.003921569}
\tikzAGCmakeSignal{iddR}{$\RLO\sigorP$}{KOLORiddR}
\newColorRGB{KOLORiddRR}{0.9647059}{0.54509807}{0.003921569}
\tikzAGCmakeSignal{iddRR}{$\RHI\sigorP$}{KOLORiddRR}
\newColorRGB{KOLORnegL}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{negL}{$\LLO\signotZ$}{KOLORnegL}
\newColorRGB{KOLORnegLL}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{negLL}{$\LHI\signotZ$}{KOLORnegLL}
\newColorRGB{KOLORnegR}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{negR}{$\RLO\signotZ$}{KOLORnegR}
\newColorRGB{KOLORnegRR}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{negRR}{$\RHI\signotZ$}{KOLORnegRR}
\newColorRGB{KOLORoneL}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{oneL}{$\LLO\sigexists$}{KOLORoneL}
\newColorRGB{KOLORoneLL}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{oneLL}{$\LHI\sigexists${KOLORoneLL}
\newColorRGB{KOLORoneR}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{oneR}{$\RLO\sigexists$}{KOLORoneR}
\newColorRGB{KOLORoneRR}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{oneRR}{$\RHI\sigexists$}{KOLORoneRR}
\newColorRGB{KOLORstoreL}{0.4392157}{0.9098039}{0.7607843}
\tikzAGCmakeSignal{storeL}{$\LLO\sigs$}{KOLORstoreL}
\newColorRGB{KOLORstoreLL}{0.4392157}{0.9098039}{0.7607843}
\tikzAGCmakeSignal{storeLL}{$\LHI\sigs$}{KOLORstoreLL}
\newColorRGB{KOLORstoreR}{0.4392157}{0.9098039}{0.7607843}
\tikzAGCmakeSignal{storeR}{$\RLO\sigs$}{KOLORstoreR}
\newColorRGB{KOLORstoreRR}{0.4392157}{0.9098039}{0.7607843}
\tikzAGCmakeSignal{storeRR}{$\RHI\sigs$}{KOLORstoreRR}
\newColorRGB{KOLORtL}{0.9647059}{0.54509807}{0.003921569}
\tikzAGCmakeSignal{tL}{$\LLO\sigtP$}{KOLORtL}
\newColorRGB{KOLORtLL}{0.9647059}{0.54509807}{0.003921569}
\tikzAGCmakeSignal{tLL}{$\LHI\sigtP$}{KOLORtLL}
\newColorRGB{KOLORtR}{0.9647059}{0.54509807}{0.003921569}
\tikzAGCmakeSignal{tR}{$\RLO\sigtP$}{KOLORtR}
\newColorRGB{KOLORtRR}{0.9647059}{0.54509807}{0.003921569}
\tikzAGCmakeSignal{tRR}{$\RHI\sigtP$}{KOLORtRR}
\newColorRGB{KOLORtrue}{0.0}{1.0}{0.0}
\tikzAGCmakeSignal{true}{$\ST\sigt$}{KOLORtrue}
\newColorRGB{KOLORtrueL}{0.0}{1.0}{0.0}
\tikzAGCmakeSignal{trueL}{$\LLO\sigt$}{KOLORtrueL}
\newColorRGB{KOLORtrueLL}{0.0}{1.0}{0.0}
\tikzAGCmakeSignal{trueLL}{$\LHI\sigt$}{KOLORtrueLL}
\newColorRGB{KOLORtrueR}{0.0}{1.0}{0.0}
\tikzAGCmakeSignal{trueR}{$\RLO\sigt$}{KOLORtrueR}
\newColorRGB{KOLORtrueRR}{0.0}{1.0}{0.0}
\tikzAGCmakeSignal{trueRR}{$\RHI\sigt$}{KOLORtrueRR}
\newColorRGB{KOLORw}{0.0}{0.0}{0.0}
\tikzAGCmakeSignal{w}{$\ST\sigwall$}{KOLORw}
\newColorRGB{KOLORx}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{x}{$\ST\sigx$}{KOLORx}
\newColorRGB{KOLORxL}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{xL}{$\LLO\sigx$}{KOLORxL}
\newColorRGB{KOLORxLL}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{xLL}{$\LHI\sigx$}{KOLORxLL}
\newColorRGB{KOLORxR}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{xR}{$\RLO\sigx$}{KOLORxR}
\newColorRGB{KOLORxRR}{0.0}{0.0}{1.0}
\tikzAGCmakeSignal{xRR}{$\RHI\sigx$}{KOLORxRR}
\newColorRGB{KOLORxoff}{0.4392157}{0.9098039}{0.7607843}
\tikzAGCmakeSignal{xoff}{$\ST\sigxoff$}{KOLORxoff}
\newColorRGB{KOLORzL}{0.95686275}{0.03137255}{0.03137255}
\tikzAGCmakeSignal{zL}{$\LLO\sigtop$}{KOLORzL}
\newColorRGB{KOLORzLL}{0.95686275}{0.03137255}{0.03137255}
\tikzAGCmakeSignal{zLL}{$\LHI\sigtop$}{KOLORzLL}
\newColorRGB{KOLORzR}{0.95686275}{0.03137255}{0.03137255}
\tikzAGCmakeSignal{zR}{$\RLO\sigtop$}{KOLORzR}
\newColorRGB{KOLORzRR}{0.95686275}{0.03137255}{0.03137255}
\tikzAGCmakeSignal{zRR}{$\RHI\sigtop$}{KOLORzRR}
\newColorRGB{KOLORzetaL}{0.99215686}{0.16470589}{0.7490196}
\tikzAGCmakeSignal{zetaL}{$\LLO\sigtopaux$}{KOLORzetaL}
\newColorRGB{KOLORzetaLL}{0.99215686}{0.16470589}{0.7490196}
\tikzAGCmakeSignal{zetaLL}{$\LHI\sigtopaux$}{KOLORzetaLL}
\newColorRGB{KOLORzetaR}{0.99215686}{0.16470589}{0.7490196}
\tikzAGCmakeSignal{zetaR}{$\RLO\sigtopaux$}{KOLORzetaR}
\newColorRGB{KOLORzetaRR}{0.99215686}{0.16470589}{0.7490196}
\tikzAGCmakeSignal{zetaRR}{$\RHI\sigtopaux$}{KOLORzetaRR}

==> Fig_New/fig___corridors_cmd.tex <==
\tikzAGCmakeSignal{ReturnllTrue}{\ensuremath{\overleftarrow{\text{T$^{\text{ll}}$}}}}{DarkGreen}%
\tikzAGCmakeSignal{ReturnllFalse}{\ensuremath{\overleftarrow{\text{F$^{\text{ll}}$}}}}{Red}%
\tikzAGCmakeSignal{SATReturnllTRUELe}{\ensuremath{\overleftarrow{\text{T$^{\text{ll}}$}}}}{DarkGreen} 	% sat:form=true:ll
\tikzAGCmakeSignal{SATReturnllFALSELe}{\ensuremath{\overleftarrow{\text{F$^{\text{ll}}$}}}}{Red} 	% sat:form=false:ll
\tikzAGCmakeSignal{SATReturnllTRUERi}{\ensuremath{\overrightarrow{\text{T$^{\text{ll}}$}}}}{DarkGreen} 	% sat:form=true:ll_sym
\tikzAGCmakeSignal{SATReturnllFALSERi}{\ensuremath{\overrightarrow{\text{F$^{\text{ll}}$}}}}{Red} 	% sat:form=false:ll_sym
\tikzAGCmakeSignal{SATValuellTrueRi}{\ensuremath{\overrightarrow{\text{t$^{\text{ll}}$}}}}{DarkGreen} 	% sat:form=true_val:ll
\tikzAGCmakeSignal{SATValuellFalseRi}{\ensuremath{\overrightarrow{\text{f$^{\text{ll}}$}}}}{Red} 	% sat:form=false_val:ll
\tikzAGCmakeSignal{SATValuellTrueLe}{\ensuremath{\overleftarrow{\text{t$^{\text{ll}}$}}}}{DarkGreen} 	% sat:form=true_val:ll_sym
\tikzAGCmakeSignal{SATValuellFalseLe}{\ensuremath{\overleftarrow{\text{f$^{\text{ll}}$}}}}{Red} 	% sat:form=false_val:ll_sym
\tikzAGCmakeSignal{SATXnllR}{\ensuremath{\overrightarrow{\text{x$_{1}^{\text{ll}}$}}}}{blue} 	% sat:form=var_1:ll
\tikzAGCmakeSignal{SATXnllL}{\ensuremath{\overleftarrow{\text{x$_{1}^{\text{ll}}$}}}}{blue} 	% sat:form=var_1:ll_sym
\tikzAGCmakeSignal{ReturnlrcTrue}{\ensuremath{\overleftarrow{\text{T$^{\text{lrc}}$}}}}{DarkGreen}%
\tikzAGCmakeSignal{ReturnlrcFalse}{\ensuremath{\overleftarrow{\text{F$^{\text{lrc}}$}}}}{Red}%
\tikzAGCmakeSignal{SATReturnlrcTRUELe}{\ensuremath{\overleftarrow{\text{T$^{\text{lrc}}$}}}}{DarkGreen} 	% sat:form=true:lrc
\tikzAGCmakeSignal{SATReturnlrcFALSELe}{\ensuremath{\overleftarrow{\text{F$^{\text{lrc}}$}}}}{Red} 	% sat:form=false:lrc
\tikzAGCmakeSignal{SATReturnlrcTRUERi}{\ensuremath{\overrightarrow{\text{T$^{\text{lrc}}$}}}}{DarkGreen} 	% sat:form=true:lrc_sym
\tikzAGCmakeSignal{SATReturnlrcFALSERi}{\ensuremath{\overrightarrow{\text{F$^{\text{lrc}}$}}}}{Red} 	% sat:form=false:lrc_sym
\tikzAGCmakeSignal{SATValuelrcTrueRi}{\ensuremath{\overrightarrow{\text{t$^{\text{lrc}}$}}}}{DarkGreen} 	% sat:form=true_val:lrc
\tikzAGCmakeSignal{SATValuelrcFalseRi}{\ensuremath{\overrightarrow{\text{f$^{\text{lrc}}$}}}}{Red} 	% sat:form=false_val:lrc
\tikzAGCmakeSignal{SATValuelrcTrueLe}{\ensuremath{\overleftarrow{\text{t$^{\text{lrc}}$}}}}{DarkGreen} 	% sat:form=true_val:lrc_sym
\tikzAGCmakeSignal{SATValuelrcFalseLe}{\ensuremath{\overleftarrow{\text{f$^{\text{lrc}}$}}}}{Red} 	% sat:form=false_val:lrc_sym
\tikzAGCmakeSignal{SATXnnlrcR}{\ensuremath{\overrightarrow{\text{x$_{2}^{\text{lrc}}$}}}}{blue} 	% sat:form=var_2:lrc
\tikzAGCmakeSignal{SATXnnlrcL}{\ensuremath{\overleftarrow{\text{x$_{2}^{\text{lrc}}$}}}}{blue} 	% sat:form=var_2:lrc_sym
\tikzAGCmakeSignal{ReturnlrTrue}{\ensuremath{\overleftarrow{\text{T$^{\text{lr}}$}}}}{DarkGreen}%
\tikzAGCmakeSignal{ReturnlrFalse}{\ensuremath{\overleftarrow{\text{F$^{\text{lr}}$}}}}{Red}%
\tikzAGCmakeSignal{SATReturnlrTRUELe}{\ensuremath{\overleftarrow{\text{T$^{\text{lr}}$}}}}{DarkGreen} 	% sat:form=true:lr
\tikzAGCmakeSignal{SATReturnlrFALSELe}{\ensuremath{\overleftarrow{\text{F$^{\text{lr}}$}}}}{Red} 	% sat:form=false:lr
\tikzAGCmakeSignal{SATReturnlrTRUERi}{\ensuremath{\overrightarrow{\text{T$^{\text{lr}}$}}}}{DarkGreen} 	% sat:form=true:lr_sym
\tikzAGCmakeSignal{SATReturnlrFALSERi}{\ensuremath{\overrightarrow{\text{F$^{\text{lr}}$}}}}{Red} 	% sat:form=false:lr_sym
\tikzAGCmakeSignal{SATValuelrTrueRi}{\ensuremath{\overrightarrow{\text{t$^{\text{lr}}$}}}}{DarkGreen} 	% sat:form=true_val:lr
\tikzAGCmakeSignal{SATValuelrFalseRi}{\ensuremath{\overrightarrow{\text{f$^{\text{lr}}$}}}}{Red} 	% sat:form=false_val:lr
\tikzAGCmakeSignal{SATValuelrTrueLe}{\ensuremath{\overleftarrow{\text{t$^{\text{lr}}$}}}}{DarkGreen} 	% sat:form=true_val:lr_sym
\tikzAGCmakeSignal{SATValuelrFalseLe}{\ensuremath{\overleftarrow{\text{f$^{\text{lr}}$}}}}{Red} 	% sat:form=false_val:lr_sym
\tikzAGCmakeSignal{SATNotlrR}{\ensuremath{\overrightarrow{\text{\ensuremath{\neg^{\text{lr}}}}}}}{Red} 	% sat:form=not:lr
\tikzAGCmakeSignal{SATNotlrL}{\ensuremath{\overleftarrow{\text{\ensuremath{\neg^{\text{lr}}}}}}}{Red} 	% sat:form=not:lr_sym
\tikzAGCmakeSignal{ReturnlTrue}{\ensuremath{\overleftarrow{\text{T$^{\text{l}}$}}}}{DarkGreen}%
\tikzAGCmakeSignal{ReturnlFalse}{\ensuremath{\overleftarrow{\text{F$^{\text{l}}$}}}}{Red}%
\tikzAGCmakeSignal{SATReturnlTRUELe}{\ensuremath{\overleftarrow{\text{T$^{\text{l}}$}}}}{DarkGreen} 	% sat:form=true:l
\tikzAGCmakeSignal{SATReturnlFALSELe}{\ensuremath{\overleftarrow{\text{F$^{\text{l}}$}}}}{Red} 	% sat:form=false:l
\tikzAGCmakeSignal{SATReturnlTRUERi}{\ensuremath{\overrightarrow{\text{T$^{\text{l}}$}}}}{DarkGreen} 	% sat:form=true:l_sym
\tikzAGCmakeSignal{SATReturnlFALSERi}{\ensuremath{\overrightarrow{\text{F$^{\text{l}}$}}}}{Red} 	% sat:form=false:l_sym
\tikzAGCmakeSignal{SATValuelTrueRi}{\ensuremath{\overrightarrow{\text{t$^{\text{l}}$}}}}{DarkGreen} 	% sat:form=true_val:l
\tikzAGCmakeSignal{SATValuelFalseRi}{\ensuremath{\overrightarrow{\text{f$^{\text{l}}$}}}}{Red} 	% sat:form=false_val:l
\tikzAGCmakeSignal{SATValuelTrueLe}{\ensuremath{\overleftarrow{\text{t$^{\text{l}}$}}}}{DarkGreen} 	% sat:form=true_val:l_sym
\tikzAGCmakeSignal{SATValuelFalseLe}{\ensuremath{\overleftarrow{\text{f$^{\text{l}}$}}}}{Red} 	% sat:form=false_val:l_sym
\tikzAGCmakeSignal{SATDisjunctionlR}{\ensuremath{\overrightarrow{\text{\ensuremath{\vee^{\text{l}}}}}}}{DarkOrange} 	% sat:form=or:l
\tikzAGCmakeSignal{SATDisjunctionlL}{\ensuremath{\overleftarrow{\text{\ensuremath{\vee^{\text{l}}}}}}}{DarkOrange} 	% sat:form=or:l_sym
\tikzAGCmakeSignal{SATDisjunctionlIdR}{\ensuremath{\overrightarrow{\text{\ensuremath{id^{\text{l}}}}}}}{DarkOrange} 	% sat:form=fct-id:l
\tikzAGCmakeSignal{SATDisjunctionlIdL}{\ensuremath{\overleftarrow{\text{\ensuremath{id^{\text{l}}}}}}}{DarkOrange} 	% sat:form=fct-id:l_sym
\tikzAGCmakeSignal{SATDisjunctionlTrueR}{\ensuremath{\overrightarrow{\text{\ensuremath{t()^{\text{l}}}}}}}{DarkOrange} 	% sat:form=fct-true:l
\tikzAGCmakeSignal{SATDisjunctionlTrueL}{\ensuremath{\overleftarrow{\text{\ensuremath{t()^{\text{l}}}}}}}{DarkOrange} 	% sat:form=fct-true:l_sym
\tikzAGCmakeSignal{ReturnrTrue}{\ensuremath{\overleftarrow{\text{T$^{\text{r}}$}}}}{DarkGreen}%
\tikzAGCmakeSignal{ReturnrFalse}{\ensuremath{\overleftarrow{\text{F$^{\text{r}}$}}}}{Red}%
\tikzAGCmakeSignal{SATReturnrTRUELe}{\ensuremath{\overleftarrow{\text{T$^{\text{r}}$}}}}{DarkGreen} 	% sat:form=true:r
\tikzAGCmakeSignal{SATReturnrFALSELe}{\ensuremath{\overleftarrow{\text{F$^{\text{r}}$}}}}{Red} 	% sat:form=false:r
\tikzAGCmakeSignal{SATReturnrTRUERi}{\ensuremath{\overrightarrow{\text{T$^{\text{r}}$}}}}{DarkGreen} 	% sat:form=true:r_sym
\tikzAGCmakeSignal{SATReturnrFALSERi}{\ensuremath{\overrightarrow{\text{F$^{\text{r}}$}}}}{Red} 	% sat:form=false:r_sym
\tikzAGCmakeSignal{SATValuerTrueRi}{\ensuremath{\overrightarrow{\text{t$^{\text{r}}$}}}}{DarkGreen} 	% sat:form=true_val:r
\tikzAGCmakeSignal{SATValuerFalseRi}{\ensuremath{\overrightarrow{\text{f$^{\text{r}}$}}}}{Red} 	% sat:form=false_val:r
\tikzAGCmakeSignal{SATValuerTrueLe}{\ensuremath{\overleftarrow{\text{t$^{\text{r}}$}}}}{DarkGreen} 	% sat:form=true_val:r_sym
\tikzAGCmakeSignal{SATValuerFalseLe}{\ensuremath{\overleftarrow{\text{f$^{\text{r}}$}}}}{Red} 	% sat:form=false_val:r_sym
\tikzAGCmakeSignal{SATXnnnrR}{\ensuremath{\overrightarrow{\text{x$_{3}^{\text{r}}$}}}}{blue} 	% sat:form=var_3:r
\tikzAGCmakeSignal{SATXnnnrL}{\ensuremath{\overleftarrow{\text{x$_{3}^{\text{r}}$}}}}{blue} 	% sat:form=var_3:r_sym
\tikzAGCmakeSignal{ReturnTrue}{\ensuremath{\overleftarrow{\text{T$^{\text{}}$}}}}{DarkGreen}%
\tikzAGCmakeSignal{ReturnFalse}{\ensuremath{\overleftarrow{\text{F$^{\text{}}$}}}}{Red}%
\tikzAGCmakeSignal{SATReturnTRUELe}{\ensuremath{\overleftarrow{\text{T$^{\text{}}$}}}}{DarkGreen} 	% sat:form=true:
\tikzAGCmakeSignal{SATReturnFALSELe}{\ensuremath{\overleftarrow{\text{F$^{\text{}}$}}}}{Red} 	% sat:form=false:
\tikzAGCmakeSignal{SATReturnTRUERi}{\ensuremath{\overrightarrow{\text{T$^{\text{}}$}}}}{DarkGreen} 	% sat:form=true:_sym
\tikzAGCmakeSignal{SATReturnFALSERi}{\ensuremath{\overrightarrow{\text{F$^{\text{}}$}}}}{Red} 	% sat:form=false:_sym
\tikzAGCmakeSignal{SATValueTrueRi}{\ensuremath{\overrightarrow{\text{t$^{\text{}}$}}}}{DarkGreen} 	% sat:form=true_val:
\tikzAGCmakeSignal{SATValueFalseRi}{\ensuremath{\overrightarrow{\text{f$^{\text{}}$}}}}{Red} 	% sat:form=false_val:
\tikzAGCmakeSignal{SATValueTrueLe}{\ensuremath{\overleftarrow{\text{t$^{\text{}}$}}}}{DarkGreen} 	% sat:form=true_val:_sym
\tikzAGCmakeSignal{SATValueFalseLe}{\ensuremath{\overleftarrow{\text{f$^{\text{}}$}}}}{Red} 	% sat:form=false_val:_sym
\tikzAGCmakeSignal{SATConjunctionR}{\ensuremath{\overrightarrow{\text{\ensuremath{\wedge^{\text{}}}}}}}{DarkPink} 	% sat:form=and:
\tikzAGCmakeSignal{SATConjunctionL}{\ensuremath{\overleftarrow{\text{\ensuremath{\wedge^{\text{}}}}}}}{DarkPink} 	% sat:form=and:_sym
\tikzAGCmakeSignal{SATConjunctionIdR}{\ensuremath{\overrightarrow{\text{\ensuremath{id^{\text{}}}}}}}{DarkPink} 	% sat:form=fct-id:
\tikzAGCmakeSignal{SATConjunctionIdL}{\ensuremath{\overleftarrow{\text{\ensuremath{id^{\text{}}}}}}}{DarkPink} 	% sat:form=fct-id:_sym
\tikzAGCmakeSignal{SATConjunctionFalseR}{\ensuremath{\overrightarrow{\text{\ensuremath{f()^{\text{}}}}}}}{DarkPink} 	% sat:form=fct-false:
\tikzAGCmakeSignal{SATConjunctionFalseL}{\ensuremath{\overleftarrow{\text{\ensuremath{f()^{\text{}}}}}}}{DarkPink} 	% sat:form=fct-false:_sym
\tikzAGCmakeSignal{SATVARR}{x$_{0}^{\text{R}}$}{blue} 	% sat:struct=var_r0
\tikzAGCmakeSignal{SATVARL}{x$_{0}^{\text{L}}$}{blue} 	% sat:struct=var_l0
\tikzAGCmakeSignal{SATVARRi}{\ensuremath{\overlineright{\text{x$_{0}$}}}}{blue} 	% sat:struct=var_builder_r0
\tikzAGCmakeSignal{SATVARLe}{\ensuremath{\overlineleft{\text{x$_{0}$}}}}{blue} 	% sat:struct=var_builder_l0
\tikzAGCmakeSignal{SATVARnR}{x$_{1}^{\text{R}}$}{blue} 	% sat:struct=var_r1
\tikzAGCmakeSignal{SATVARnL}{x$_{1}^{\text{L}}$}{blue} 	% sat:struct=var_l1
\tikzAGCmakeSignal{SATVARnRi}{\ensuremath{\overlineright{\text{x$_{1}$}}}}{blue} 	% sat:struct=var_builder_r1
\tikzAGCmakeSignal{SATVARnLe}{\ensuremath{\overlineleft{\text{x$_{1}$}}}}{blue} 	% sat:struct=var_builder_l1
\tikzAGCmakeSignal{SATVARnnR}{x$_{2}^{\text{R}}$}{blue} 	% sat:struct=var_r2
\tikzAGCmakeSignal{SATVARnnL}{x$_{2}^{\text{L}}$}{blue} 	% sat:struct=var_l2
\tikzAGCmakeSignal{SATVARnnRi}{\ensuremath{\overlineright{\text{x$_{2}$}}}}{blue} 	% sat:struct=var_builder_r2
\tikzAGCmakeSignal{SATVARnnLe}{\ensuremath{\overlineleft{\text{x$_{2}$}}}}{blue} 	% sat:struct=var_builder_l2
\tikzAGCmakeSignal{SATVARnnnR}{x$_{3}^{\text{R}}$}{blue} 	% sat:struct=var_r3
\tikzAGCmakeSignal{SATVARnnnL}{x$_{3}^{\text{L}}$}{blue} 	% sat:struct=var_l3
\tikzAGCmakeSignal{SATVARnnnRi}{\ensuremath{\overlineright{\text{x$_{3}$}}}}{blue} 	% sat:struct=var_builder_r3
\tikzAGCmakeSignal{SATVARnnnLe}{\ensuremath{\overlineleft{\text{x$_{3}$}}}}{blue} 	% sat:struct=var_builder_l3


==> Fig_New/x.tex <==
\relax 
\@setckpt{../denys.tex}{
\setcounter{page}{1}
\setcounter{equation}{0}
\setcounter{enumi}{0}
\setcounter{enumii}{0}
\setcounter{enumiii}{0}
\setcounter{enumiv}{0}
\setcounter{footnote}{0}
\setcounter{mpfootnote}{0}
\setcounter{part}{0}
\setcounter{section}{0}
\setcounter{subsection}{0}
\setcounter{subsubsection}{0}
\setcounter{paragraph}{0}
\setcounter{subparagraph}{0}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{parentequation}{0}
}


==> vocabulary.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% FOR APPENDIX
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \newcommand{\SigL}{\text{\textsf{L}}}
% \newcommand{\SigR}{\text{\textsf{R}}}
% \newcommand{\SigT}{\text{\textsf{T}}}
% \newcommand{\SigF}{\text{\textsf{F}}}
\newcommand{\SigB}{\text{\textsf{B}}}
\tikzAGCmakeSignal{TRi}{\ensuremath{\overrightarrow{\text{T}}}}{DarkGreen}
\tikzAGCmakeSignal{FRi}{\ensuremath{\overrightarrow{\text{F}}}}{DarkGreen}
\tikzAGCmakeSignal{TLe}{\ensuremath{\overleftarrow{\text{T}}}}{DarkGreen}
\tikzAGCmakeSignal{FLe}{\ensuremath{\overleftarrow{\text{F}}}}{DarkGreen}
\tikzAGCmakeSignal{SuccessRi}{\ensuremath{\overrightarrow{\text{success}}}}{DarkGreen}
\tikzAGCmakeSignal{StoreSuccessLe}{\ensuremath{\overleftarrow{\text{T$^{\emptyset}$}}}}{DarkGreen}
\tikzAGCmakeSignal{StoreFailureRi}{\ensuremath{\overrightarrow{\text{F$^{\emptyset}$}}}}{Red}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% MIDDLE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\tikzAGCmakeSignal{Wall}{w}{Black}

\tikzAGCmakeSignal[,line width=.1em,dotted]{Div}{\ensuremath{\overrightarrow{\text{div}}}}{Red}
\tikzAGCmakeSignal[,line width=.1em,dashed]{Lo}{\ensuremath{\overrightarrow{\text{lo}}}}{DarkOrange}
\tikzAGCmakeSignal[,line width=.1em,dotted]{Hi}{\ensuremath{\overrightarrow{\text{hi}}}}{DeepPurple}
\tikzAGCmakeSignal[,line width=.1em,dashed]{Back}{\ensuremath{\overleftarrow{\text{back}}}}{Blue}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% COMB
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tikzAGCmakeSignal{SATVARN}{x$_{n}$}{blue} 	% sat:struct=var_r0
\tikzAGCmakeSignal{SATVAR}{x$_{0}$}{blue} 	% sat:struct=var_r0
\tikzAGCmakeSignal{SATVARn}{x$_{1}$}{blue} 	% sat:struct=var_r0
\tikzAGCmakeSignal{SATVARnn}{x$_{2}$}{blue} 	% sat:struct=var_r0
\tikzAGCmakeSignal{SATVARnnn}{x$_{3}$}{blue} 	% sat:struct=var_r0
\tikzAGCmakeSignal{SATVARR}{x$_{0}$}{blue} 	% sat:struct=var_r0
\tikzAGCmakeSignal{SATVARnR}{x$_{1}$}{blue} 	% sat:struct=var_r0
\tikzAGCmakeSignal{SATVARnnR}{x$_{2}$}{blue} 	% sat:struct=var_r0
\tikzAGCmakeSignal{SATVARnnnR}{x$_{3}$}{blue} 	% sat:struct=var_r0
\tikzAGCmakeSignal{SATVARL}{x$_{0}$}{blue} 	% sat:struct=var_r0
\tikzAGCmakeSignal{SATVARnL}{x$_{1}$}{blue} 	% sat:struct=var_r0
\tikzAGCmakeSignal{SATVARnnL}{x$_{2}$}{blue} 	% sat:struct=var_r0
\tikzAGCmakeSignal{SATVARnnnL}{x$_{3}$}{blue} 	% sat:struct=var_r0
%
\tikzAGCmakeSignal{SATVARi}{x$_{i}$}{blue} 	% sat:struct=var_r0
\tikzAGCmakeSignal{SATVARip}{x$_{i+1}$}{blue} 	% sat:struct=var_r0
%
\tikzAGCmakeSignal{Start}{\ensuremath{\overrightarrow{\text{start}}}}{Blue}
\tikzAGCmakeSignal{StartLo}{\ensuremath{\overrightarrow{\text{start$_{\text{lo}}$}}}}{Blue}
%
\tikzAGCmakeSignal{ArmLeLe}{\ensuremath{\overleftarrow{\text{a}}}}{DarkGrey}
\tikzAGCmakeSignal{ArmRiRi}{\ensuremath{\overrightarrow{\text{a}}}}{DarkGrey}
%
\tikzAGCmakeSignal{MakeZeroLe}{\ensuremath{\overleftarrow{\text{m$_0$}}}}{ColorGENERATEDZero}
\tikzAGCmakeSignal{MakeOneLe}{\ensuremath{\overleftarrow{\text{m$_1$}}}}{ColorGENERATEDone}
\tikzAGCmakeSignal{MakeTwoLe}{\ensuremath{\overleftarrow{\text{m$_2$}}}}{ColorGENERATEDtwo}
\tikzAGCmakeSignal{MakeThreeLe}{\ensuremath{\overleftarrow{\text{m$_3$}}}}{ColorGENERATEDthree}
%
\tikzAGCmakeSignal{MakeZeroRi}{\ensuremath{\overrightarrow{\text{m$_0$}}}}{ColorGENERATEDZero}
\tikzAGCmakeSignal{MakeOneRi}{\ensuremath{\overrightarrow{\text{m$_1$}}}}{ColorGENERATEDone}
\tikzAGCmakeSignal{MakeTwoRi}{\ensuremath{\overrightarrow{\text{m$_2$}}}}{ColorGENERATEDtwo}
\tikzAGCmakeSignal{MakeThreeRi}{\ensuremath{\overrightarrow{\text{m$_3$}}}}{ColorGENERATEDthree}
%
\tikzAGCmakeSignal{MakeILe}{\ensuremath{\overleftarrow{\text{m$_{{i}}$}}}}{ColorGENERATEDthree}
\tikzAGCmakeSignal{MakeIpOneLe}{\ensuremath{\overleftarrow{\text{m$_{{i+1}}$}}}}{ColorGENERATEDthree}
\tikzAGCmakeSignal{MakeNLe}{\ensuremath{\overleftarrow{\text{m$_{n}$}}}}{ColorGENERATEDthree}
\tikzAGCmakeSignal{MakeIRi}{\ensuremath{\overrightarrow{\text{m$_{{i}}$}}}}{ColorGENERATEDthree}
\tikzAGCmakeSignal{MakeIpOneRi}{\ensuremath{\overrightarrow{\text{m$_{{i+1}}$}}}}{ColorGENERATEDthree}
\tikzAGCmakeSignal{MakeNRi}{\ensuremath{\overrightarrow{\text{m$_{n}$}}}}{ColorGENERATEDthree}%
\tikzAGCmakeSignal{BottomLeft}{b$_{\text{l}}$}{Blue}
\tikzAGCmakeSignal{BottomRight}{b$_{\text{r}}$}{Blue}
%
\tikzAGCmakeSignal{StoreRi}{\ensuremath{\overrightarrow{\text{store}}}}{Black}
\tikzAGCmakeSignal{StoreLe}{\ensuremath{\overleftarrow{\text{store}}}}{Black}
\tikzAGCmakeSignal{Success}{T}{DarkGreen}
\tikzAGCmakeSignal{SuccessLe}{\ensuremath{\overleftarrow{\text{success}}}}{DarkGreen}
\tikzAGCmakeSignal{StoreSuccess}{\ensuremath{\overrightarrow{\text{T$^{\emptyset}$}}}}{DarkGreen}
\tikzAGCmakeSignal{StoreFailure}{\ensuremath{\overleftarrow{\text{F$^{\emptyset}$}}}}{Red}
\tikzAGCmakeSignal{CollectRi}{\ensuremath{\overrightarrow{\text{collect}}}}{cyan}
\tikzAGCmakeSignal{CollectLe}{\ensuremath{\overleftarrow{\text{collect}}}}{cyan}
%
\tikzAGCmakeSignal[,line width=.1em,dotted]{FailureRi}{\ensuremath{\overrightarrow{\text{Fail}}}}{Red}
\tikzAGCmakeSignal[,line width=.1em,dotted]{FailureLe}{\ensuremath{\overleftarrow{\text{Fail}}}}{Red}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\tikzAGCmakeSignal{FormStartR}{$\phi_{\text{R}}$}{DarkGrey}
\tikzAGCmakeSignal{FormStartL}{$\phi_{\text{L}}$}{DarkGrey}
\tikzAGCmakeSignal{FormStartWall}{$\phi_{\text{W}}$}{DarkGrey}

\tikzAGCmakeSignal{SplitterRight}{s$_{\text{r}}$}{Blue}

\newrgbcolor{ColorGENERATEDZero}{0.0 0.25098039215686274 1.0}
\newrgbcolor{ColorGENERATEDone}{0.0 0.5490196078431373 1.0}
\newrgbcolor{ColorGENERATEDtwo}{0.0 0.8509803921568627 1.0}
\newrgbcolor{ColorGENERATEDthree}{0.0 1.0 0.8509803921568627}

%\tikzAGCmakeSignal{MakeNpOneLe}{\ensuremath{\overleftarrow{\text{m$_{\text{n+1}}$}}}}{ColorGENERATEDthree}
%\tikzAGCmakeSignal{MakeNpOneRi}{\ensuremath{\overrightarrow{\text{m$_{\text{n+1}}$}}}}{ColorGENERATEDthree}

